CheXpercept: A Benchmark for Evaluating Expert-Level Lesion Perception in Chest X-rays

The evaluation of vision-language models (VLMs) for chest X-ray (CXR) analysis has largely been limited to disease-presence classification without visual grounding. Such evaluations fail to verify the expert-level lesion perception necessary to ensure the clinical reliability of VLMs. To address these limitations, we introduce CheXpercept, a sequential, multi-level perception benchmark that mirrors a radiologist's cognitive workflow across coarse-level detection, fine-level contour evaluation and revision, and semantic-level attribute extraction. To ensure high clinical fidelity at scale, we construct the dataset using a semi-automated generation pipeline paired with a review by six medical experts. CheXpercept contains 10,400 QA items derived from 2,100 CXRs, covering seven clinically critical pulmonary and cardiac lesions. To demonstrate the current landscape of VLM perception, we benchmark 14 general and medical VLMs on CheXpercept. The models achieve adequate performance only at the coarse level, with accuracy degrading precipitously on deeper visual tasks. Notably, medical VLMs show almost no perceptual advantage over their general-domain counterparts, highlighting a systemic flaw in current domain adaptation. The code and dataset will be publicly available.

==> table/results_stage3.tex <==
% Stage 3 sub-task accuracy (Oracle-Passed).
% Only Revision-Required path is applicable (Stage 3 exists only on RR).
% TODO: fill proprietary rows when evaluations complete.

\begin{table}[t]
\centering
\caption{Stage 3 sub-task accuracy (\%) on the Revision-Required path under the Oracle-Passed setting. Point-Wise Revision is split into \emph{Expansion} and \emph{Contraction}; \emph{Revision Result} is the single-choice selection over four candidate masks. Best within each group is bolded.}
\label{tab:results_stage3}
\small
\setlength{\tabcolsep}{6pt}
\begin{tabular}{@{}l ccc@{}}
\toprule
\textbf{Model} & \textbf{Expansion} & \textbf{Contraction} & \textbf{Revision Result} \\
\midrule
\multicolumn{4}{l}{\textit{Proprietary}} \\
GPT-5.4                         & -- & -- & -- \\
GPT-5.4-nano                    & -- & -- & -- \\
Gemini-3.1-pro                  & -- & -- & -- \\
Gemini-3.1-Flash                & -- & -- & -- \\
\midrule
\multicolumn{4}{l}{\textit{General (open-source)}} \\
Qwen3.6-27B              & 12.1 & 29.1 & 35.7 \\
Qwen3.5-122B             & 7.4 & 29.3 & 35.3 \\
GLM-4.6V                 & 8.1 & \textbf{43.3} & 31.1 \\
InternVL3.5-38B          & 4.0 & 15.4 & 33.9 \\
Gemma4-31B               & 5.6 & \textbf{45.9} & \textbf{54.7} \\
\midrule
\multicolumn{4}{l}{\textit{Medical (open-source)}} \\
MedGemma-27B                      & 1.9 & \textbf{31.1} & 25.9 \\
MedGemma1.5-4B                    & 0.0 & 0.0 & 25.4 \\
HuatuoGPT-Vision-7B               & 0.0 & 5.9 & 22.4 \\
Lingshu-32B                       & 0.0 & \textbf{37.1} & 22.4 \\
Hulu-Med-32B                      & 5.3 & 2.1 & 24.9 \\
\bottomrule
\end{tabular}
\end{table}


==> table/results_stage4.tex <==
% Stage 4 sub-task accuracy (Oracle-Passed), aggregated over RR + RF paths.
% Cardiomegaly has no Stage 4 and is excluded from these aggregates by the analysis script.
% TODO: fill proprietary rows when evaluations complete.

\begin{table}[t]
\centering
\caption{Stage 4 sub-task accuracy (\%) aggregated over the Revision-Required and Revision-Free paths under the Oracle-Passed setting. Cardiomegaly is excluded as its semantic attributes are not applicable. Best within each group is bolded.}
\label{tab:results_stage4}
\small
\setlength{\tabcolsep}{6pt}
\begin{tabular}{@{}l cccc@{}}
\toprule
\textbf{Model} & \textbf{Distribution} & \textbf{Location} & \textbf{Severity} & \textbf{Comparison} \\
\midrule
\multicolumn{5}{l}{\textit{Proprietary}} \\
GPT-5.4                         & -- & -- & -- & -- \\
GPT-5.4-nano                    & -- & -- & -- & -- \\
Gemini-3.1-pro                  & -- & -- & -- & -- \\
Gemini-3.1-Flash                & -- & -- & -- & -- \\
\midrule
\multicolumn{5}{l}{\textit{General (open-source)}} \\
Qwen3.6-27B              & 60.1 & 56.1 & 45.6 & 66.5 \\
Qwen3.5-122B             & 67.3 & \textbf{55.4} & 61.3 & 71.1 \\
GLM-4.6V                 & \textbf{71.2} & 36.9 & 65.0 & 79.2 \\
InternVL3.5-38B          & \textbf{71.8} & 38.2 & \textbf{67.9} & \textbf{80.6} \\
Gemma4-31B               & 62.4 & \textbf{64.7} & 65.9 & 59.5 \\
\midrule
\multicolumn{5}{l}{\textit{Medical (open-source)}} \\
MedGemma-27B                      & \textbf{45.7} & 30.8 & 35.6 & \textbf{68.6} \\
MedGemma1.5-4B                    & 28.2 & 17.0 & 15.3 & 17.8 \\
HuatuoGPT-Vision-7B               & 35.3 & 27.8 & 36.9 & 10.3 \\
Lingshu-32B                       & \textbf{48.9} & \textbf{41.0} & \textbf{48.3} & \textbf{79.0} \\
Hulu-Med-32B                      & \textbf{52.5} & 39.8 & 42.1 & 38.8 \\
\bottomrule
\end{tabular}
\end{table}

